Well-conditioned ultraspherical and spectral integration methods for resolvent analysis of channel flows of Newtonian and viscoelastic fluids

Modal and nonmodal analyses of fluid flows provide fundamental insight into the early stages of transition to turbulence. Eigenvalues of the dynamical generator govern temporal growth or decay of individual modes, while singular values of the frequency response operator quantify the amplification of disturbances for linearly stable flows. In this paper, we develop well-conditioned ultraspherical and spectral integration methods for frequency response analysis of channel flows of Newtonian and viscoelastic fluids. Even if a discretization method is well-conditioned, we demonstrate that calculations can be erroneous if singular values are computed as the eigenvalues of a cascade connection of the frequency response operator and its adjoint. To address this issue, we utilize a feedback interconnection of the frequency response operator with its adjoint to avoid computation of inverses and facilitate robust singular value decomposition. Specifically, in contrast to conventional spectral collocation methods, the proposed method (i) produces reliable results in channel flows of viscoelastic fluids at high Weissenberg numbers ($\sim 500$); and (ii) does not require a staggered grid for the equations in primitive variables.

==> figure2.tex <==
\begin{picture}(21,7)(-4,-1)
\linethickness{0.2mm}
\multiput(1,0)(4,0){1}%
{\line(1,0){10}}
\multiput(3,0)(4,0){1}%
{\line(0,1){2.5}}
\multiput(1,2.5)(4,0){1}%
{\line(1,0){10}}
\multiput(0.8,1.25)(4,0){1}%
{\vector(0,1){0.9}}
\multiput(0.8,1.25)(4,0){1}%
{\vector(1,0){0.9}}
\multiput(0.8,1.25)(4,0){1}%
{\vector(-2,-3){0.4}}
\put(0.4,2.3){$y$}
\put(1.4,1.5){$x$}
\put(-0.05,0.7){$z$}
\put(2.0,-0.5){\small Poiseuille}
\put(2.5,-1){\small flow}
\put(7.0,-0.5){\small Couette}
\put(7.5,-1){\small flow}
\qbezier(3,0)(7.5,1.25)(3,2.5)
%\put(10,0){\line(2,1){2.5}}
% \put(10,2.5){\line(2,-1){2.5}}
 \put(3,0.2){\vector(1,0){0.7}}
 \put(3,0.4){\vector(1,0){1.15}}
 \put(3,0.6){\vector(1,0){1.6}}
 \put(3,0.8){\vector(1,0){2}}
 \put(3,1){\vector(1,0){2.2}}
 \put(3,1.2){\vector(1,0){2.3}}
 \put(3,1.4){\vector(1,0){2.2}}
 \put(3,1.6){\vector(1,0){2.1}}
 \put(3,1.8){\vector(1,0){1.8}}
 \put(3,2){\vector(1,0){1.4}}
 \put(3,2.2){\vector(1,0){1}}
 \put(3,2.4){\vector(1,0){0.4}}
 \qbezier(5,3)(9.5,4.25)(5,5.5)
 \put(5,3.2){\vector(1,0){0.7}}
 \put(5,3.4){\vector(1,0){1.15}}
 \put(5,3.6){\vector(1,0){1.6}}
 \put(5,3.8){\vector(1,0){2}}
 \put(5,4){\vector(1,0){2.2}}
 \put(5,4.2){\vector(1,0){2.3}}
 \put(5,4.4){\vector(1,0){2.2}}
 \put(5,4.6){\vector(1,0){2.1}}
 \put(5,4.8){\vector(1,0){1.8}}
 \put(5,5){\vector(1,0){1.4}}
 \put(5,5.2){\vector(1,0){1}}
 \put(5,5.4){\vector(1,0){0.4}}
%\put(10.5,0){\vector(0,1){2.5}}
%\put(10.5,2.5){\vector(0,-1){2.5}}
%\put(10.8,1.25){$2h$}
\put(3,2.5){\line(2,3){2}}
\put(3,0){\line(2,3){2}}
\put(5,3){\line(0,1){2.5}}
\put(5,3){\line(0,1){2.5}}
\put(1,2.5){\line(2,3){2}}
\put(11,2.5){\line(2,3){2}}
\put(3,5.5){\line(1,0){10}}
\put(11,0){\line(2,3){2}}
\put(1,0){\line(2,3){2}}
\put(3,3){\line(1,0){10}}
\put(8,2.5){\line(2,3){2}}
\put(8,0){\line(2,3){2}}
\put(10,3){\line(0,1){2.5}}
\put(8,0){\line(0,1){2.5}}
\put(6.75,0){\line(1,1){2.5}}
\put(8.75,3){\line(1,1){2.5}}
\put(8,0.1){\vector(-1,0){1.2}}
\put(8,0.3){\vector(-1,0){1.0}}
\put(8,0.5){\vector(-1,0){0.8}}
\put(8,0.7){\vector(-1,0){0.6}}
\put(8,0.9){\vector(-1,0){0.4}}
\put(8,1.1){\vector(-1,0){0.2}}
%\put(8,1.3){\vector(1,0){0.1}}
\put(8,1.5){\vector(1,0){0.25}}
\put(8,1.7){\vector(1,0){0.45}}
\put(8,1.9){\vector(1,0){0.65}}
\put(8,2.1){\vector(1,0){0.85}}
\put(8,2.3){\vector(1,0){1.05}}
\put(8,2.5){\vector(1,0){1.25}}

\put(10,3.1){\vector(-1,0){1.2}}
\put(10,3.3){\vector(-1,0){1.0}}
\put(10,3.5){\vector(-1,0){0.8}}
\put(10,3.7){\vector(-1,0){0.6}}
\put(10,3.9){\vector(-1,0){0.4}}
\put(10,4.1){\vector(-1,0){0.2}}
%\put(8,1.3){\vector(1,0){0.1}}
\put(10,4.5){\vector(1,0){0.25}}
\put(10,4.7){\vector(1,0){0.45}}
\put(10,4.9){\vector(1,0){0.65}}
\put(10,5.1){\vector(1,0){0.85}}
\put(10,5.3){\vector(1,0){1.05}}
\put(10,5.5){\vector(1,0){1.25}}
 \put(3,0.4){\vector(1,0){1.15}}
 \put(3,0.6){\vector(1,0){1.6}}
 \put(3,0.8){\vector(1,0){2}}
 \put(3,1){\vector(1,0){2.2}}
%\put(4,3){\line(0,1){2.5}}
%\put(2,0){\line(0,1){2.5}}
\end{picture}


==> tikz_common_styles.tex <==
%_______________________________________________________________
%
%     Tikz_common_styles
%
%     TikZ styles for drawing block diagrams.
%
%      Roy Smith,  15 July 2014
%
%_______________________________________________________________
\typeout{Reading Tikz styles:  tikz_common_styles}
%
%   Block diagram styles
% added by MJ
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
%
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=1.0cm,
                                top color=blue!10, bottom color=blue!10]%
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]%
\tikzstyle{connector} = [->,thick]%
\tikzstyle{line} = [thick]%
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]%
\tikzstyle{guide} = []%
%
%   colours for various blocks
\tikzstyle{deltablock} = [block, top color=red!10, bottom color=red!10]%
\tikzstyle{controlblock} = [block, top color=green!10, bottom color=green!10]%
\tikzstyle{weightblock} = [block, top color=orange!10, bottom color=orange!10]%
\tikzstyle{clpblock} = [block, top color=cyan!10, bottom color=cyan!10]%
%
%  styles for dimming block components.
\tikzstyle{block_dim} = [draw,rectangle,thick,minimum height=2em,minimum width=2em,
                                color=black!15]%
\tikzstyle{sum_dim} = [draw,circle,inner sep=0mm,minimum size=2mm,color=black!15]%
\tikzstyle{connector_dim} = [->,thick,color=black!15]%
%
%    Graph styles
\tikzstyle{smalllabel} = [font=\footnotesize]%
\tikzstyle{axiswidth}=[semithick]%
\tikzstyle{axiscolor}=[color=black!50]%
\tikzstyle{help lines} =[color=blue!40,very thin]%
\tikzstyle{axes} = [axiswidth,axiscolor,<->,smalllabel]%
\tikzstyle{axis} = [axiswidth,axiscolor,->,smalllabel]%
\tikzstyle{tickmark} = [thin,smalllabel]%
\tikzstyle{plain_axes} = [axiswidth,smalllabel]%
\tikzstyle{w_axes} = [axiswidth,->,smalllabel]%
\tikzstyle{m_axes} = [axiswidth,smalllabel]%
\tikzstyle{dataplot} = [thick]%
%
%_______________________________________________________________

